Simultaneous Safe Screening of Features and Samples in Doubly Sparse Modeling

The problem of learning a sparse model is conceptually interpreted as the process of identifying active features/samples and then optimizing the model over them. Recently introduced safe screening allows us to identify a part of non-active features/samples. So far, safe screening has been individually studied either for feature screening or for sample screening. In this paper, we introduce a new approach for safely screening features and samples simultaneously by alternatively iterating feature and sample screening steps. A significant advantage of considering them simultaneously rather than individually is that they have a synergy effect in the sense that the results of the previous safe feature screening can be exploited for improving the next safe sample screening performances, and vice-versa. We first theoretically investigate the synergy effect, and then illustrate the practical advantage through intensive numerical experiments for problems with large numbers of features and samples.

==> App/appC.tex <==
\section{Other experiments}
\label{app:other-experiments}
In this appendix, we show the rest of the experimental results.
\begin{figure}[htbp]
  \begin{center}
   \subfigure{\includegraphics[clip,width=4.0cm]{./Fig/regression/bar_rcv1-train_1}}
   \subfigure{\includegraphics[clip,width=4.0cm]{./Fig/regression/bar_real-sim_1}}
   % \subfigure{\includegraphics[clip,width=4.0cm]{./Fig/regression/bar_E2006-train_20000}}
   \caption{Total computation time for training 100 solutions for various values of $\lambda$ in regression problems.}
    \label{fig:acc_time_regression_app}
  \end{center}
\end{figure}

\begin{figure}[htbp]
  \begin{center}
   \subfigure{\includegraphics[clip,width=7.0cm]{./Fig/classification/itr_time_0205_gisette_scale}}
   \subfigure{\includegraphics[clip,width=7.0cm]{./Fig/classification/itr_time_0205_rcv1-train}}
   % \subfigure{\includegraphics[clip,width=7.0cm]{./Fig/classification/itr_time_real-sim}}
   % \subfigure{\includegraphics[clip,width=7.0cm]{./Fig/classification/itr_time_rcv1-test}}
   \caption{Number of optimization steps and computation time in classification problems ({\tt rcv1-train} and {\tt rcv1-train} datasets).
   See the caption in \figurename~\ref{fig:per_itr_time_classification_spdc_rcv1_test}.}
   \label{fig:per_itr_time_classification_spdc_app}
  \end{center}
\end{figure}



\begin{figure*}[t]
  \begin{center}
   \includegraphics[clip,width=17cm]{./Fig/classification/0205_rate2_gisette_scale}\\
   \includegraphics[clip,width=17cm]{./Fig/classification/0205_rate2_rcv1-train}\\
   % \includegraphics[clip,width=15cm]{./Fig/classification/0203_rate2_real-sim}\\
   %\includegraphics[clip,width=15cm]{./Fig/classification/0205_rate2_rcv1-test}
   \caption{Safe screening and keeping rates in classification problems ({\tt rcv1-train} and {\tt rcv1-train} datasets). See the caption in \figurename~\ref{fig:screeing_rate_smoothed_hinge}.}
   \label{fig:screeing_rate_smoothed_hinge_app}
  \end{center}
\end{figure*}




\begin{figure*}[t]
  \begin{center}
   \includegraphics[clip,width=17cm]{./Fig/regression/0205_rate2_rcv1-train}
   \includegraphics[clip,width=17cm]{./Fig/regression/0205_rate2_real-sim}
   % \subfigure{\includegraphics[clip,width=18cm]{./Fig/regression/0203_rate2_E2006-train_20000}}
   \caption{Safe screening and keeping rates in regression problems. See the caption in \figurename~\ref{fig:screeing_rate_smoothed_hinge}.}
   \label{fig:screeing_rate_smoothed_insensitive_app}
  \end{center}
\end{figure*}


==> App/fig_tab.tex <==
% figures and tables

% ------------------------- Fig1 -------------------------

% ------------------------- Fig2 -------------------------

% ------------------------- Fig3 -------------------------

% ------------------------- Fig4 -------------------------


